Reviving Any-Subset Autoregressive Models with Principled Parallel Sampling and Speculative Decoding

In arbitrary-order language models, it is an open question how to sample tokens in parallel from the correct joint distribution. With discrete diffusion models, the more tokens they generate in parallel, the less their predicted distributions adhere to the originally learned data distribution, as they rely on a conditional independence assumption that only works with infinitesimally small timesteps. We find that a different class of models, any-subset autoregressive models (AS-ARMs), holds the solution. As implied by the name, AS-ARMs can generate tokens in any order, and in parallel. Moreover, AS-ARMs support parallelized joint probability density estimation, allowing them to correct their own parallel-generated token distributions, via our Any-Subset Speculative Decoding (ASSD) algorithm. ASSD provably enables generation of tokens from the correct joint distribution, with the number of neural network calls upper bounded by the number of tokens predicted. We empirically verify that ASSD speeds up language generation, without sacrificing quality. Furthermore, we provide a mathematically justified scheme for training AS-ARMs for generation, and show that AS-ARMs achieve state-of-the-art performance among sub-200M parameter models on infilling benchmark tasks, and nearly match the performance of models 50X larger on code generation. Our theoretical and empirical results indicate that the once-forgotten AS-ARMs are a promising direction of language modeling.

==> old_intro.tex <==
\section{Introduction}

%\se{i would remove the bold paragraph header}

%\noindent\textbf{Motivation:}
%We are in the era of LLMs, with models like GPT \cite{achiam2023gpt}, LLaMA \cite{touvron2023llama}, DeepSeek \cite{liu2024deepseek}, Gemini \cite{team2023gemini}, and Claude penetrating into ubiquitous societal use. 
Almost all the commonly used LLMs \cite{achiam2023gpt, touvron2023llama, liu2024deepseek, team2023gemini} are autoregressive, \textit{i.e.}, they only support left-to-right token generation. 
However, in many important tasks (\textit{e.g.}, code completion, story infilling, biological data analysis), left-to-right generation is not an efficient approach, as the arbitrary conditional distributions are not tractable. 
%While this is a reasonable inductive bias for human language, there are other discrete domains in which this is not a reasonable inductive bias, \textit{e.g.}, code, DNA and protein sequences. 
Thus, we want discrete-space generative models that can generate in any order, not just left-to-right. 
%\se{i would rephrase slightly, it's not a matter of inductive bias, it's more an issue of efficiency (those conditional distributions are not tractable)}

%\noindent\textbf{Current SoTA:} 
A current solution in SoTA autoregressive models is training the model to do causal prediction on permuted documents (prefix-suffix-middle) \cite{bavarian2022efficient, fried2022incoder, roziere2023code}. While this works, it is heuristic, and not guaranteed to adhere to the correct structure (\textit{e.g.}, if a specific number of tokens is required). 
%\se{inefficient would be something like gibbs sampling. for the prompting approach, the right adjective is heuristic, and potentially incorrect}
%\se{same comment as above, ar has a principled way but it's inefficient}
As an alternative solution, researchers have recently introduced discrete diffusion models \cite{lou2023discrete, sahoo2024simple, gong2024scaling, austin2021structured}, which can inherently generate tokens in arbitrary order. Furthermore, they support sampling of multiple tokens in parallel per network evaluation, in contrast to autoregressive models being able to generate only one token per network evaluation. This parallelism can provide significant speedups \cite{lou2023discrete}. %\se{cite}
%\se{say this parallelism is good for speed}

%\textcolor{red}{the more parallelized you want, the closer to the mean field. mean field means independent prediction by position}

%\noindent\textbf{Limitations of SoTA:} 
However, a major limitation of the parallel token generation in discrete diffusion models is that the more tokens that are generated in parallel (\textit{i.e.}, taking large discretized timestep $\Delta t$ in the reverse process), the closer to the mean field approximation their distributions become. This is because the predictions at each position are made with a conditional independence assumption, as detailed in Section \ref{sec:sampling_strat}. So, unless they are generated one by one (\textit{i.e.}, the limit with $\Delta t \rightarrow 0$), they do not adhere to the limiting joint density distribution as learned by the model during training. 
%\se{true is a bit imprecise. maybe limiting? or learned during training? basically the do come from some joint, it's just not the "right" one}
Thus, while parallel sampling improves speed, it is theoretically and empirically known to degrade quality \cite{lou2023discrete}.

%\noindent\textbf{Desired Improvements to SoTA:} 
If we were able to generate multiple tokens in parallel that adhere to the true joint density distribution, we could greatly increase the speed of generative models, without degrading quality. Currently, a mathematically principled solution does not exist for arbitrary-order models. %; the only available solutions degrade quality as speed increases \cite{sahoo2024simple, lou2023discrete, deschenaux2024beyond}.
However, speculative decoding techniques recently provided a solution for autoregressive models. Speculative decoding works similarly to rejection sampling, in that a cheap draft model predicts the next few tokens in a sequence, and they are either accepted or rejected by the oracle model, depending on the draft distribution's fidelity to the oracle distribution. Importantly, the outputted distribution is provably the same as would have been obtained from sampling only from the expensive oracle model, while usually requiring fewer neural network forward passes \cite{chen2023accelerating, leviathan2023fast}. We take inspiration from the success of speculative decoding for autoregressive models, hoping to translate its benefits to arbitrary-order models.

%\noindent\textbf{Goal and Solution:} 
\textbf{\textit{Thus, we wish to design discrete-space (\textit{i.e.}, language) models that support: (1) arbitrary-order generation; (2) principled parallel token generation from the joint distribution.}} Towards this goal, we revive 
a class of generative models we call \textit{Any-Subset Autoregressive Models (\asarm)} \cite{yang2019xlnet, shih2022training} and combine them with recent advances in speculative decoding techniques to create a principled paradigm of parallelized arbitrary-order language generation. 
%\se{it might be a good idea to pitch this as any subset instead of any order}
\asarm can generate tokens in any order (which easily breeds parallel generation), and they inherently support probability density estimation. We prove in Section \ref{sec:any_order_speculative_decoding} that the ability to do density estimation allows \asarm to correct the tokens generated in parallel such that they adhere to the true joint distribution, via a scheme similar to speculative decoding. Furthermore, our proposed \textit{Any-Subset Speculative Decoding (\assd)} algorithm is mathematically guaranteed to never increase the number of neural network evaluations, which means that it can only speed up generation without losing quality.

%\noindent\textbf{Results:} 
We empirically verify that \assd speeds up generation while maintaining the correct joint distribution, matching our theoretical analysis. We also show that appropriately trained \asarm (particularly XLNet \cite{yang2019xlnet}) outperform diffusion and autoregressive models on infilling benchmarks, while needing fewer parameters and training resources. \footnote{Models available at \href{https://huggingface.co/therealgabeguo/AO-ARM-generative}{https://huggingface.co/therealgabeguo/AO-ARM-generative}.} 

\se{i feel like the logic of the argument is a bit convoluted. how about: AR is sota, but can be slow and can't do infilling. these are 2 main ways to do infilling: any order and discrete diffusion. any order is accurate but slow. diffusion is potentially fast but inaccurate.. we propose}

% In summary, our contributions are:
% \begin{itemize}
%     \item We introduce \textit{Any-Order Speculative Decoding}, which provides a principled way to generate tokens in parallel in arbitrary orders besides left-to-right. It provably produces tokens from the correct joint distribution, and is mathematically guaranteed never to increase the number of model evaluations.
%     \item We introduce an effective and mathematically justified training recipe to convert AO-ARMs into generative models. \textcolor{red}{let's release the model on Huggingface. Code is too messy atm.}
%     \item We provide empirical evidence that AO-ARMs can outperform autoregressive and discrete diffusion paradigms in certain benchmark tasks, while using fewer training resources and smaller model sizes. This revives a recently overlooked paradigm of language modeling research.
% \end{itemize}
